Bandit Pareto Set Identification: the Fixed Budget Setting

We study a multi-objective pure exploration problem in a multi-armed bandit model. Each arm is associated to an unknown multi-variate distribution and the goal is to identify the distributions whose mean is not uniformly worse than that of another distribution: the Pareto optimal set. We propose and analyze the first algorithms for the \emph{fixed budget} Pareto Set Identification task. We propose Empirical Gap Elimination, a family of algorithms combining a careful estimation of the ``hardness to classify'' each arm in or out of the Pareto set with a generic elimination scheme. We prove that two particular instances, EGE-SR and EGE-SH, have a probability of error that decays exponentially fast with the budget, with an exponent supported by an information theoretic lower-bound. We complement these findings with an empirical study using real-world and synthetic datasets, which showcase the good performance of our algorithms.

==> parts/analysis.tex <==
\section{THEORETICAL GUARANTEES}
We present in this section a generic analysis of some gap-based elimination algorithms for Pareto set identification in the fixed-budget setting. The goal is to identify the Pareto set given a budget $T$: using at most $T$ samples minimize the probability of mis-identification of the Pareto set. 
Let $\bX_{a,s}$ denote the $s$-th observation drawn \iid from distribution $\nu_a$. Let further define for any arm $a$ and at any round $r$, $\vmuh_a(r) := T_a(r)^{-1}\sum_{s=1}^{T_a(r)} \bX_{a, s}$ where $T_a(r)$ is the number of times arm $a$ has been played up to the end of round $r$ and 
\begin{eqnarray*}
	\mh(i,j; r) &:=& \min_{d}[\muh_j^d(r) -  \muh_i^d(r)], \\
	\Mh(i,j; r) &:=& \| (\vmuh_i(r) - \vmuh_j(r))^+\|_2. 
	\end{eqnarray*}
	Letting $A_r$ denote the set of arms still active at the beginning of round $r$, we define 	the empirical Pareto set of the active arms: 
\begin{eqnarray*}S_r &:=& \{i \in A_r : \nexists j \in A_r : \vmuh_i(r) \prec \vmuh_j(r) \},\\
 & = &\{i \in A_r: \forall j  \in A_r \backslash \{i\}, \Mh(i,j;r) > 0 \}\;.
\end{eqnarray*}

We also define for any arm $i \in A_r$ the empirical quantities
\begin{eqnarray*}
\widehat \Delta_{i, r}^\star &:=& \max_{j\in A_r\backslash\{ i\}}\mh(i,j;r), \\
\widehat \delta_{i,r}^\star &:=& \min_{j \in A_r \backslash\{i\}} [\Mh(i,j;r) \;\land\; (\Mh(j,i;r)^+ + (\widehat \Delta_{i, r}^\star)^+)]
\end{eqnarray*}
 and for any $i\in A_r$
\begin{eqnarray}
\label{eq:def-emp-gap}
	\widehat \Delta_{i,r} := \begin{cases}
		\widehat \Delta_{i, r}^\star & \text{ if } i \in A_r \backslash{S_r},\\
		\widehat\delta_{i,r}^\star & \text{ else. }
	\end{cases}
\end{eqnarray}
The algorithm proceeds by elimination of an (or a set of) arm(s)  in each phase: this arm classified as optimal or sub-optimal. At the end the algorithm recommends the arms classified as optimal as the Pareto set. We propose a generic analysis depending on the generic parameters $\bm \lambda, \bm t$. As a consequence, we further derive the analysis of two algorithms inspired from the allocation schemes of Successive~Rejects \citep{audibert_best_2010} and Sequential~Halving \citep{karnin_almost_2013}.
\subsection{Generic analysis}
 Let $R>0$ be a number of rounds and $\lambda_1 \dots, \lambda_{R+1}$ be a non-increasing sequence of numbers in $[K]$ such that 
\begin{equation}
\label{eq:cond1}
\lambda_1 = K \quad \text{and}\quad \lambda_{R+1} \in \{0, 1\}. 
\end{equation}
Letting $T>0$ denote the total budget of the algorithm, we define a sequence of integers $\{t_1,\dots, t_R\}$ such that 
\begin{equation}
\label{eq:cond2}
\sum_{r=1}^R \lambda_r t_r \leq T,	
\end{equation}
and ideally with an equality.   For any round  $r\in [R]$, we define 
$$ n_r = \sum_{s= 1}^r t_s, $$
which is the total numbers of pulls of each survival arm in round $r$. 
In the sequel we denote by $\bm t$ and $\bm \lambda$ the sequences $\{t_r\}$ and $\{\lambda_r\}$. 

\begin{algorithm}
\caption{Generic Gap-Based Elimination}\label{alg:three}
\KwResult{Pareto set}
\KwData{parameters $\bm t, \bm \lambda$}
\Input{Set $A_1 = \{1, \dots, K\}, B_1 := \emptyset$, $D_1 = \emptyset$} 
 \For{$r=1, 2, \dots, R$}{

  \Sample each arm $a \in A_r$ for $t_{r}$ rounds
  
  \textbf{let} $A_{r+1}$ be the set of $\lambda_{r+1}$ arms in $A_r$ with the smallest empirical gaps $\widehat\Delta$
  
 \tcp{ties broken by removing empirically sub-optimal arms}
 
 $ B_{r+1} \gets B_r \cup \{ S_r \cap (A_r \backslash A_{r+1})\}$ \; 
 
 $ D_{r+1} \gets D_r \cup \{  (A_r \backslash A_{r+1}) \backslash S_r \}$ \; 
 
 }
 \Output{$\widehat S = B_{R+1}  \cup A_{R+1}$}
\end{algorithm}





Letting $(\cdot)$ be the permutation such that $\Delta_{(1)}\leq \dots\leq \Delta_{(K)}$, 
we define for any bandit $\bm\nu$\begin{eqnarray*}
   H(\nu) &:=& H_1(\nu):= \sum_{i=1}^K \Delta_i^{-2}\\
   H_2(\nu) &:=& \max_{i \in [K]} i \Delta_{(i)}^{-2}. 
\end{eqnarray*}
We ease notation and write $H, H_2$ when the instance $\nu$ is clear from the context. 
We introduce: 
$$ H_3^{\bm t, \bm \lambda}  := \min_{r\in [R]} n_r\Delta_{(\lambda_{r+1} +1)}^2,$$
which depends on the allocation schemes and will be shown to be of order $T/(H_2\log K)$ for Successive~Rejects and Sequential~Halving. 
We state the main result of this section on the probability of error $e_T(\nu)$. 
\begin{restatable}{theorem}{mainRes}
\label{thm:main-res}
Let $T\geq 2K$ and $\nu$ be a bandit with multivariate $\sigma$-subgaussian arms. Then 
 the probability of error of \autoref{alg:three} for PSI satisfies
 $$ e_T(\nu) \leq K R 5^D \exp\left( - \frac{H_3^{\bm t, \bm\lambda}}{800\sigma^2}) \right).$$
 \end{restatable}
 This result shows that the probability of failure of \autoref{alg:three} decreases exponentially fast with the quantity $H_3^{\bm t, \bm \lambda}$, which will be shown to be proportional to $T/H_2$ the allocation schemes studied in the sequel.  
\subsection{Successive Rejects}
\autoref{alg:three} can be specialized in the same fashion of SR, that is we proceed by an elimination of one arm in each round. So we set $R= K-1$. For any $r\in [K-1]$ we define 
$\lambda_r = K+1-r$, $$\eps_r = \left\lceil  \frac{1}{\overline{\log (K)}} \frac{T-K}{K+1-r}\right\rceil$$ and finally 
$$ t_r = \eps_{r} - \eps_{r-1},$$
with $\eps_0 := 0$ and $\overline{\log (K)} := 2^{-1} +\sum_{i=2}^{K}i^{-1}$. Then  \begin{eqnarray*}
	\sum_{r=1}^{K-1}t_r\lambda_r &=& \sum_{r=1}^{K-1}(\eps_r - \eps_{r-1})(K+1-r),\\
	&=& 2\eps_{K-1}  + \sum_{r=1}^{K-1}\eps_{r-1} \; \text{(telescoping)},\\
	&\leq& T,
\end{eqnarray*}
where the last inequality follows from the proof of SR(section 4 of \cite{audibert_best_2010}). Therefore, both sequences $\{t_r\}$ and $\{\lambda_{r}\}$ satisfies the conditions aforementioned.
\begin{proposition}
	\label{thm:sr}
	Let  $T\geq 2K$ and $\nu$ be a bandit with $\sigma$-subgaussian marginals. Then 
 the probability of error of \autoref{alg:three} run with $\bm t_{\textrm{SR}}$ and $\bm \lambda_{\textrm{SR}}$ satisfies 
 $$ e_T(\nu) \leq K(K-1)5^D\exp\left( - \frac{T-K}{800\sigma^2H_2\overline\log(K)}\right).$$
\end{proposition}
\begin{proof}
This is a simple application of \autoref{thm:main-res}. It remains to compute $H_3^{\bm t_{\textrm{SR}}, \bm\lambda_{\textrm{SR}}}$. We have $n_r= \sum_{s=1}^r (\eps_s - \eps_{s-1}) = \eps_r$, $\lambda_{r+1}^{\textrm{SR}} +1= K+1-r$, so 
	\begin{eqnarray*}
		H_3^{\bm t_{\textrm{SR}}, \bm\lambda_{\textrm{{SR}}}}  &:=& \min_{r\in [K-1]} n_r\Delta_{(\lambda_{r+1} +1)}^2,\\
		&\geq& \min_{r\in [K-1]} \frac{\Delta_{(K+1-r)}^2}{\overline{\log (K)}} \frac{T-K}{K+1-r},\\
		&=& \frac{T-K}{\overline \log (K)} \frac{1}{\max_{r\in \{2,\dots K\}}r\Delta_{(r)}^{-2}}\\
		&=& \frac{T-K}{\overline \log (K)} \frac{1}{H_2}. 
	\end{eqnarray*}
\end{proof}

\subsection{Sequential Halving}
This algorithm, proceeds in $R=\lceil\log_2(K)\rceil$ rounds. Let $\lambda_1 = K$ and for any $r\in \{1,\dots, \lceil\log_2(K)\rceil\}$, 
$$ \lambda_{r+1} := \lceil \lambda_r/2\rceil \; \text{and}\; t_r := \left\lfloor \frac{T}{\lvert A_r \lvert \lceil\log_2(K)\rceil } \right\rfloor. $$
It is simple to show that $\lambda_{\lceil\log_2(K)\rceil +1} = 1$. We 
easily verify that $\{\lambda_r\}$ and $\{t_r\}$  satisfy the assumption xx, so \autoref{thm:main-res} applies. 
We derive the following result for SH. 


\begin{proposition}
	\label{thm:sh}
	Let $c<1/16$, $T\geq 2K$ and $\nu$ be a bandit with $\sigma$-subgaussian marginals. Then 
 the probability of error of \autoref{alg:three} run with $\bm t_{\textrm{SH}}$ and $\bm \lambda_{\textrm{SH}}$ satisfies 
 $$ e_T(\nu) \leq K \lceil\log_2(K)\rceil 5^D\exp\left( - \frac{T}{1600\sigma^2 H_2 \lceil\log_2(K)\rceil}\right).$$
\end{proposition}

\begin{proof}
We compute $H_3^{\bm t_{\textrm{SH}}, \bm\lambda_{\textrm{SH}}}$ and we derive the result using \autoref{thm:main-res}. 
We have $n_r^\textrm{SH} := \sum_{s=1}^r t_s^\textrm{SH} \geq  \frac{T}{\lambda_r^\textrm{SH} \lceil\log_2(K)\rceil}$ and $\lambda_r^\textrm{SH}\leq  2(\lambda_{r+1}^\textrm{SH} +1)$.  
	Then 
	\begin{eqnarray*}
		H_3^{\bm t_{\textrm{SH}}, \bm\lambda_{\textrm{SH}}}  &:=& \min_{r\in \{1, \dots, \lceil\log_2(K)\rceil\}} n_r^\textrm{SH}\Delta_{(\lambda_{r+1}^\textrm{SH} +1)}^2, \\
	&\geq& \min_{r\in \{1, \dots, \lceil\log_2(K)\rceil\}} \frac{\Delta_{(\lambda_{r+1}^\textrm{SH}+1)}^2 }{\lambda_{r+1}^\textrm{SH} +1 } \times \frac{T}{2\lceil\log_2(K)\rceil},\\
	&=& \frac{T/(2\lceil\log_2(K)\rceil)}{\max_{r\in \lvert\lceil\log_2(K)\rceil\lvert} (\lambda_{r+1}^{\textrm{SH}}+1) \Delta_{(\lambda_{r+1}^{\textrm{SH}}+1)}^{-2}}\\
	&\geq& \frac{T}{2H_2 \lceil\log_2(K)\rceil}. 
	\end{eqnarray*}
The result then follows by application of \autoref{thm:main-res}. 
\end{proof}
This result improves upon the {Successive~Rejects} instanciation in the polynomial dependence ($K\log_2(K)$ instead of $K^2$). 
However, we see in the experiments that both algorithms have pretty close performance (likewise in BAI, \cite{karnin_almost_2013}). Recall that when $D=1$, PSI is exactly \emph{best arm identification}. Compared to the analysis Sequential~Halving for BAI (\cite{karnin_almost_2013}), we have an extra polynomial $K$ factor.  
This is due to the fact that our proof uses a good event which holds for any arm. Unlike \cite{karnin_almost_2013} we allow all the samples collected so far to be used (no re-starting). To our knowledge, this is the first analysis of {Sequential Halving} without \emph{re-starting} in BAI (although it is long known that it performs very well without re-starting).    

\subsection{Sketch of proof} 
 We define for any arm $i$ and round $r$ the event
 $$ \xi(i; r) := \left\{\left \|(\vmuh_{i, n_r} - \vmu_i -  \right\|_2 \leq c \Delta_{(\lambda_{r+1} +1)}\right\} $$ 
 and for any $c>0$, 
$$ \cE_c^1 := \bigcap_{r\in [R]}\bigcap_{i \in [K]}\;  \xi(i; r) .$$ Note that $\cE_c^1$ depends on the sequences $\{t_r\}$ and $\{\lambda_r\}$. 
The idea of the proof is to show that \autoref{alg:three} does not make any error on the event $\cE_c^1$.  

For any sub-optimal arm $i$, breaking ties arbitrarily, let $i^\star := \argmax_{j\in \cS^\star} \m(i, j)$, which by definition yields $\Delta_i = \m(i, i^\star)$. For a sub-optimal arm $i$, we know that $i^\star \in \cS$ always exists. Moreover, this arm could be the unique arm dominating the arm $i$. Therefore it is important to ensure that $i$ is no longer active because before removing $i^\star$, otherwise $i$ could appear as optimal w.r.t the remaining active arms.  
We state below an important concentration result which is only valid under the assumption that $i^\star$  is active whenever $i$ is active. 

\begin{restatable}{lemma}{lemGapIneq}
\label{lem:lem-gap-ineq} Assume that the event $\cE_c^1$ holds. Let $r\in [R]$ and assume that for \emph{any} sub-optimal arm $j \in A_r$, $j^\star \in A_r$. Then, for any sub-optimal arm $i\in A_r$,
	$$\lvert \widehat \Delta_{i, r}^\star - \Delta_i^\star \lvert \leq 2c\Delta_{(\lambda_{r+1}+1)} $$
	and for any optimal arm $i \in A_r$, $$ \widehat \delta_{i,r}^\star \geq \Delta_i -4c \Delta_{(\lambda_{r+1} +1)}.$$
\end{restatable}

This result permits to prove the following crucial property for \autoref{alg:three}: arm $i^\star$ is indeed never deactivated before arm $i\in (\cS^\star)^\complement$.  
\begin{restatable}{lemma}{lemref}\label{lem:lemref} Let $c < 1/10$. 
	On the event $\cE_c^1$, for any $r\in [R+1]$ and for any sub-optimal arm $i$, if $i\in A_r$ then $i^\star \in A_r$. In particular, arm $i^\star$ cannot be deactivated before arm $i$. 
\end{restatable} 
As a consequence of \autoref{lem:lemref}, if $A_{R+1}$ contains one arm and $\cE_c^1$ holds, then this arm is optimal. 

Using \autoref{lem:lem-gap-ineq} and \autoref{lem:lemref}, we show that for $c<1/10$, if $\cE_c^1$ holds, then $\widehat S = \cS^\star$. \autoref{thm:main-res} 
 then follows by upper-bounding the probability of $\bar{\cE_c^1}$ using Hoeffding's inequality. 


 
 
\subsection{Discussion}
\autoref{thm:sr} and  \autoref{thm:sh} show that the probability of error of both the Successive Rejects and Sequential Halving instanciations decrease exponentially fast with $T/(H_2\log(K))$. Similar results have been obtained for many single-objective pure exploration problems in the fixed-budget setting (see e.g \cite{audibert_best_2010, karnin_almost_2013, locatelli_optimal_2016}).   
Using \autoref{thm:main-res}, we can easily derive an upper bound on the the probability of error of the uniform allocation strategy. We set $ R=1, \lambda_2 = 0, t_1 = n_1=  T/K$ which is indeed the uniform allocation. It follows that $H_3^{\bm t, \bm \lambda} =  n_1\Delta_{(\lambda_2 +1)}^2 = T/(K\Delta_{(1)}^{-2})$ and
thus the probability of error of the uniform allocation satisfies
\begin{equation}
\label{eq:prob-ua}
e_T(\nu) \leq 2K5^D\exp\left( - \frac{c^2T}{800\sigma^2 (K\Delta_{(1)}^{-2})}\right).	
\end{equation}
We remark that the decay factor in the exponential is larger for the Successive Rejects and Sequential Halving instanciations, in particular when $K$ is large. 
However, when all the gaps are of the same order, i.e $\Delta_1 \approx \dots\approx \Delta_K$ we have $K\Delta_{(1)}^{-2}\approx H_2\approx H$  and Equation \eqref{eq:prob-ua} becomes, 
$$ e_T(\nu) \leq 2K5^D\exp\left( - \frac{c^2T}{800\sigma^2 H }\right),	 $$
which is better than both Successive Rejects and Sequential Halving.  It is known in BAI \citep{audibert_best_2010}, the uniform allocation strategy is optimal in the fixed-budget when the sub-optimality gaps are all close.  
\begin{table}
	\centering
	\begin{tabular}{|c|c|}
		\hline
Algorithm & Mis-identification probability\\
\hline
SR. & $K^2D\exp\left(-T/(H_2\log K)\right)$\\\hline 
SH. & $ K\log(K)D \exp\left(-T/(H_2\log K)\right)$\\\hline 
Uniform Alloc. & $KD \exp\left(-T/(K \Delta_{(1)}^{-2})\right)$\\\hline
	\end{tabular}
	\caption{Different algorithms and upper-bounds (up to constants) on $e_T(\nu)$.}
\end{table}

\paragraph{Relation to BAI} When $D=1$, PSI is equivalent to BAI. In this case, at any round $r$, $S_r = \{\widehat a_r\}$ reduces to the empirical best arm. From Equation~\ref{eq:def-emp-gap} we have for any $i\neq\widehat a_r$, 
$$ \widehat \Delta_{i, r} = \muh_{\widehat a_r, r} - \muh_{i, r}$$
and $$\widehat \Delta_{\widehat a_r, r} = \min_{i\in A_r\backslash\{\widehat a_r\}} \widehat \Delta_{i, r}.$$
Then, our tie-breaking rule ensures that no arm is accepted before the last round and at each round $r$, the $\lambda_{r+1}$ arms with the largest empirical means are kept and the final survival arm is recommended as optimal. Therefore, when $D=1$, our instanciations of Successive~Rejects and Sequential~Halving matches their original definition for BAI. 






==> parts/lower_bound.tex <==
%\subsection{Lower bound}
We present in this section a lower-bound for some class of instances. %Let $\bm\Theta = (\vmu_1 \dots \vmu_K)^\T$. %For an instance $\nu$, let $\cD(\nu) = [K]\setminus\cS^\star(\nu).$ 
Denoting by $\Omega(i):= \{j\in [K]:\vmu_i \prec \vmu_j \}$ the set of arms that dominate arm $i$, we define $\cB$ to be the set of means $\bm\Theta$ such that: (1): for any $i\in \cS^\star, \exists\;  \underline i$ such that $\Omega(\underline i) = \{ i\}$ and $\Delta_i = \Delta^\star_{\underline i}$; (2): for any $i\in \cD, \exists d_i\in [D]$ such that $\tilde \theta := (\mu_i^1, \dots , \mu_i^{d_i}+ \Delta_i^\star, \dots, \mu_i^D)$ is optimal w.r.t $\{ \vmu_1, \dots, \vmu_K\}$. 

Let  $\nu:= (\nu_1, \dots, \nu_K)$ be an instance whose means $\bm\Theta \in \cB$ and such that $\nu_i \sim \cN(\vmu_i, \sigma^2 I)$. For every $i\in [K]$ we define the alternative instance $ \nu^{(i)} := (\nu_1, \dots \nu_i^{(i)}, \dots, \nu_K)$ in which only arm $i$ is modified:
\begin{equation}
	\vmu_i^{(i)} := \begin{cases}
		\vmu_i - 2\Delta_i e_{d_{\underline i}} & \text{ if } i \in \cS^\star(\nu) ,\\
		\vmu_i + 2\Delta_i e_{d_i}&\text{ else },
	\end{cases}
\end{equation}
where $e_1,\dots, e_D$ denotes the canonical basis of $\bR^D$. We prove the following.

\begin{restatable}{theorem}{thmLbdConsistent}
\label{thm:thm-lbd-consistent} 
Let $\bm\Theta:=(\vmu_1 \dots \vmu_K)^\T \in \cB$ and $\nu:=(\nu_1, \dots, \nu_K)$ where $\nu_i \sim \cN(\vmu_i, \sigma^2I)$. For any algorithm $\cA$, there exists $i\in [K]$ such that %$ H(\nu^i) \leq  H(\nu)$ and 
$$ \max(e_T^{\cA}(\nu^{(i)}), e_T^{\cA}(\nu)) \geq \exp\left( - \frac{2T}{\sigma^2 H(\nu)}\right).$$ 
\end{restatable}

In Appendix~\ref{sec:lowerBound} we further prove that there exists $\bm\Theta \in \cB$ such that for all $i\in [K]$, $H(\nu^{(i)}) \leq H(\nu)$\todoem{Say more?}, hence there exists some instances $\widetilde{\nu}$ (either $\nu$ or one of the $\nu^{(i)}$'s) such that $e_T^{\cA}(\tilde{\nu}) \geq \exp\left( - {2T}/({\sigma^2 H(\widetilde{\nu})})\right)$. On such instances, the decay rate of EGE-SR and EGE-SH is optimal up to constants factors and $\log(K)$ terms, and that of APE-FB is optimal up to constant factors, when the complexity is known. 
%In Appendix~\ref{sec:lowerBound} we prove a more general lower-bound that holds for any instance. 

%$$ \forall i, j \in \cS^\star, \M(i,j)\geq 4 \max(\Delta_{\underline i}^\star, \Delta_{\underline j}^\star).$$ 


